ChatCAD+: Towards a Universal and Reliable Interactive CAD using LLMs

The integration of Computer-Aided Diagnosis (CAD) with Large Language Models (LLMs) presents a promising frontier in clinical applications, notably in automating diagnostic processes akin to those performed by radiologists and providing consultations similar to a virtual family doctor. Despite the promising potential of this integration, current works face at least two limitations: (1) From the perspective of a radiologist, existing studies typically have a restricted scope of applicable imaging domains, failing to meet the diagnostic needs of different patients. Also, the insufficient diagnostic capability of LLMs further undermine the quality and reliability of the generated medical reports. (2) Current LLMs lack the requisite depth in medical expertise, rendering them less effective as virtual family doctors due to the potential unreliability of the advice provided during patient consultations. To address these limitations, we introduce ChatCAD+, to be universal and reliable. Specifically, it is featured by two main modules: (1) Reliable Report Generation and (2) Reliable Interaction. The Reliable Report Generation module is capable of interpreting medical images from diverse domains and generate high-quality medical reports via our proposed hierarchical in-context learning. Concurrently, the interaction module leverages up-to-date information from reputable medical websites to provide reliable medical advice. Together, these designed modules synergize to closely align with the expertise of human medical professionals, offering enhanced consistency and reliability for interpretation and advice. The source code is available at https://github.com/zhaozh10/ChatCAD.

==> alg/MSD.tex <==
% % % =====================================
% \RestyleAlgo{ruled}
% \begin{algorithm}
% \caption{LLM-based knowledge retrieval}\label{alg:MSD}
% \begin{lstlisting}[language=Python]
% # infobase: Tree-like nested dictionary
% # query: User's text input
% # bot: A LLM-based chatbot
% # Initialize chatbot via task-specific prompt
% bot.init()
% # Store the information that LLM has searched
% info_stack=[]
% # Topics of interest
% all_topics=infobase.keys()
% related_topics=kNN(query,all_topics)
% info_stack.push(related_topics)
% response=bot.get_needed_topic(related_topics)
% while True:
%     # LLM finds related knowledge
%     if response is ``found'':
%         # LLM returns founded knowledge
%         found_data=bot.get_info()
%         return found_data
%     # LLM finds nothing related
%     elif response is ``no_choice'':
%         # Backtracking
%         info_stack.pop()
%         # Retrieval end up in failure
%         if len(info_stack)==0:    
%             return None
%         # Get parent topic as next topic
%         next_item_dict=info_stack.top()
%         related_topics=prompt(next_item_dict)
%     # LLM chooses a topic
%     elif response in related_topics:
%         # Get chosen topic as next topic
%         this_item_dict=info_stack.top()
%         next_item_dict=now_item_dict[response]
%         # Push next information into the stack
%         info_stack.push(next_item_dict)
%         # Prompt LLM to choose from topic list
%         related_topics=prompt(next_item_dict)
%     # Get LLM's next choice
%     response=bot.get_needed_topic(related_topics)
% \end{lstlisting}
% \end{algorithm}
% % =====================================
 

% % =====================================
\RestyleAlgo{ruled}
\begin{algorithm}
\caption{LLM-based knowledge retrieval}\label{alg:MSD}
\begin{lstlisting}[language=Python]
# infobase: Tree-like dictionary
# info_stack: A stack store history information
# query: User's text input
# bot: A LLM-based chatbot
# prompt(): Present topics to be selected

all_topics=list(infobase.keys())
# topics of interest
related_topics=kNN(query,all_topics)
info_stack.push(related_topics)
response=bot.get_needed_topic(related_topics)
while True:
    # terminate 
    if response == "found":
        found_knowledge=bot.get_info()
        return found_knowledge
    # backtrack
    elif response == "no choice":
        info_stack.pop()
        next_item_dict=info_stack.top()
    # select a valid topic
    elif response in related_topics:
        this_item_dict=info_stack.top()
        next_item_dict=now_item_dict[response]
        info_stack.push(next_item_dict)
    related_topics=prompt(next_item_dict)
    response=bot.get_needed_topic(related_topics)
\end{lstlisting}
\end{algorithm}
% =====================================

==> alg/knowledge_retri.tex <==
% \def\SetClass{article}
% \documentclass{\SetClass}
% \usepackage[lined,boxed,commentsnumbered]{algorithm2e}
% \begin{document}
% \begin{algorithm}[H]
% \caption{Simulation-optimization heuristic}\label{algorithm}
%   \SetAlgoLined
%   \KwIn{input: query $q$; nested dictionary $infobase$}
%   \KwOut{related knowledge}

%   {special treatment for initialize prompt}\;
%   \While{True}{
%     current\_topic$\leftarrow$query\_stack.top()\;
%     current\_prompt$\leftarrow$generatePrompt(q, current\_topic)\;
%     now\_res$\leftarrow$getResFromChatbot(current\_prompt)\;
%     \If{now\_res is $found$}{
%        answer$\leftarrow$getAnswerFromChatbot()\;
%        return answer\;
%     }
% 		\ElseIf{now\_res is $not\_found$}{
%       query\_stack.pop()\;
%       \If{query\_stack is $empty$}{
% 	      return $Not found!$;
%       }
%     }
% 		\ElseIf{now\_res is a legal subtopic}{
%       next\_topic$\leftarrow$current\_topic.getSubtopic(now\_res)\;
%       query\_stack.push(next\_topic)\;
%     }
%   }
%   \caption{LLM-based knowledge retrieval}
% \end{algorithm}
% \end{document}

% \def\SetClass{article}
% \documentclass{\SetClass}

\begin{algorithm}
\SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Find}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined
  \KwIn{user query $q$, knowledge database $\mathbf{D}$}
  \KwOut{related knowledge $k$}
  \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
  % topics$\leftarrow$\FindCompress{$\mathbf{D}$}\
  % topics$\leftarrow$text2vec($q$,$\mathbf{D}\textrm{.keys}$)

  {Initialize}\;
  \While{True}{
    current\_topic$\leftarrow$query\_stack.top()\;
    current\_prompt$\leftarrow$generatePrompt(q, current\_topic)\;
    now\_res$\leftarrow$getResFromChatbot(current\_prompt)\;
    \If{now\_res is $found$}{
       answer$\leftarrow$getAnswerFromChatbot()\;
       return answer\;
    }
		\ElseIf{now\_res is $not\_found$}{
      query\_stack.pop()\;
      \If{query\_stack is $empty$}{
            break;
      }
    }
		\ElseIf{now\_res is a legal subtopic}{
      next\_topic$\leftarrow$current\_topic.getSubtopic(now\_res)\;
      query\_stack.push(next\_topic)\;
    }
  }
  \caption{LLM-based knowledge retrieval}\label{alg:know_ret}
\end{algorithm}


==> tables/illustration_knowledgeengine.tex <==

\begin{table*}
    \begin{tabular}{|p{\textwidth}|}
        \hline
    \textbf{User query:} Is pleural effusion serious? \\
    \hline
    \textbf{System prompt (Round 1):} 
    I want you to play the role of a virtual librarian. Now, you must search the knowledge base for medical knowledge that is most likely to be helpful to the patient. I will play the role of the knowledge base, providing you with medical knowledge and searchable topics. You need to choose a search topic from the options I provide, and I will provide you with new medical knowledge and new searchable topics. Please repeat this process until you believe that the medical knowledge you obtained from me may be helpful to the patient's question. At that point, please let me know, "The librarian has found it." The patient's question is: "Is pleural effusion serious?" You should try to search for knowledge related to this question. Now, you must choose one topic option from the following that is most likely to be helpful and reply to me with its name: '\textbf{Atelectasis},' '\textbf{Pleural Effusion},' '\textbf{Mediastinal Mass},' '\textbf{Aspiration Pneumonia},' '\textbf{Community-Acquired Pneumonia},' '\textbf{Hospital-Acquired Pneumonia},' '\textbf{Ventilator-Associated Pneumonia},' '\textbf{Pneumothorax},' '\textbf{Pulmonary Edema},' '\textbf{Chronic Obstructive Pulmonary Disease (COPD)},' '\textbf{pleural Fibrosis and Calcification}.'  Please note that you are not allowed to answer the patient's question, provide any other content, give advice, explain your selection, or make any assumptions. You are only allowed to choose a topic to query from the options provided. Only reply with the name of the topic you want to search.
  \\
    \hline
    \textbf{LLM (Round 1): Pleural Effusion.} 
\\
    \hline
    \textbf{System prompt (Round 2):} 
    Well done! The medical knowledge you retrieved is: \textbf{\{the abstract section of pleural effusion\}}.
    If you believe that you have found medical knowledge that may be helpful for the question "Is pleural effusion severe?" please reply with 'The librarian has found it.' If not, you must choose one of the following topic options that is most likely to be helpful and reply to me with its name: '\textbf{Etiology},' '\textbf{Symptoms and Signs},' '\textbf{Diagnosis},' '\textbf{Treatment},' '\textbf{The librarian needs more information.}' Only reply with the name of the option you want to search, no need to provide any other content. \\
    \hline
    \textbf{LLM (Round 2):} \textbf{Symptoms and Signs}. 
    \\
    \hline
    \textbf{System prompt (Round 3):} Well done! The medical knowledge you retrieved is as follows: \textbf{\{the ``Symptoms and Signs'' section of Pleural effusion\}} If you believe that the medical knowledge you have retrieved is helpful in answering the question "Is pleural effusion serious?" \textbf{please reply with 'The librarian found it.'} \textbf{If not, you must reply with 'The librarian needs additional information.'} Just reply with the name of the option you wish to query; there is no need to reply with any other content.\\
    \hline
    \textbf{LLM (Round 3):} \textbf{The librarian found it.} \\
    \hline
    \textbf{System prompt (Round 4):} 
    Please tell me which medical knowledge you just retrieved that might be helpful for the question "Is pleural effusion serious?" \textbf{Print the text within the ''' without printing any other content.}\\
    \hline
    \textbf{LLM (Round 4):}
\textbf{\{the ``Symptoms and Signs'' section of Pleural effusion\}}
    \\
    \hline
    \end{tabular}
    \caption{Illustration of the process of LLM-based knowledge retrieval. The system prompt will ask the LLM to find most related knowledge from a given list of medical topics recursively. Once the LLM does not find needed knowledge in round 3, the system prompt will backtrack from section-level to topic-level, and ask it to begin a new round of selection.}
    \label{tab:illustration_knowledge}
\end{table*} 

==> tables/interactionQA.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lcccccccccc}
    \toprule
          & ACC   & PRE   & C-BLEU & BLEU-1 & BLEU-2 & BLEU-3 & BLEU-4 & ROUGE-1 & ROUGE-2 & ROUGE-L \\
    \midrule
    ChatGLM2 & 0.435 & 0.454 & 2.43  & 4.903 & 3.303 & 2.141 & 1.607 & 25.178 & 12.169 & 11.396 \\
    ChatGLM2+Ours & 0.465 & 0.500 & 7.93  & 13.542 & 8.317 & 5.801 & 4.302 & 40.470 & 19.742 & 18.957 \\
    ChatGLM3 & 0.458 & 0.473 & 3.27  & 4.773 & 3.021 & 2.149 & 1.62  & 39.153 & 19.330 & 16.915 \\
    ChatGLM3+Ours & 0.472 & 0.524 &       & 12.636 &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:interactionQA}%
\end{table}%


==> tables/retrieval_cmp/retrieval_cmp.tex <==
% \newcommand{\tred}[1]{\textcolor{red}{#1}}
% \newcommand{\tgrn}[1]{\textcolor{ForestGreen}{#1}}
% \newcommand{\tblu}[1]{\textcolor{MidnightBlue}{#1}}
% \newcommand{\tpurp}[1]{\textcolor{DarkOrchid}{#1}}

\begin{CJK*}{UTF8}{gbsn}
\begin{table*}
  \begin{tabular}{|p{\textwidth}|}
    \hline
    \textbf{Q1} 牙周炎怎么治？只吃药就够了吗？ \\
    \hline
    \textbf{{K1 (Baseline)}} \tred{食管癌可在年轻时发生。Unna-Thost病和Vorner病：常染色体显性遗传。Papillon-Lefèvre综合征：常染色体隐性遗传，出生后6个月之内发病。严重牙周炎可能导致牙齿脱落。Vohwinkel综合征：常染色体显性遗传，患者可发生进行性趾（指）断症和高频听力损失。弥漫性非表皮松解性掌跖角化病：这种常染色体显性遗传形式在婴儿期发展，引起界限分明的对称性角化病，累及整个手掌和脚底。", "治疗": \{ "概述": " 对症治疗 对症措施可以包括 润肤剂 、 角质剥脱剂 和物理方法去除。} \\
    \hline
    \textbf{K1 (Ours)} 治疗危险因素 洁治和龈下刮治 \tgrn{必要时口服抗生素，将抗生素缓释剂置于牙周袋内，或全身用药与局部用药相结合} 手术处理或拔除患牙 治疗\tgrn{可控制的危险因素，如口腔卫生不良、糖尿病和吸烟，改善预后}。 对于所有的牙周炎，第一阶段治疗包括彻底的洁治、龈下刮治和根面处理（通过根面平整祛除病灶或毒素影响的牙骨质和牙本质）以祛除菌斑和沉积的牙结石，必须加强日常的口腔卫生。彻底的家庭口腔卫生是必要的，包括仔细刷牙和使用牙线来帮助清洁。使用洗必泰棉签或冲洗。医生应该教病人如何执行这些步骤。3周后重新评估患者。如果此时牙周袋深度不超过4毫米，则只需定期清洁即可。有时制作一瓣牙周袋组织允许给牙根更深部位实行刮治和根面平整术。 \tgrn{如果存在深牙周袋，可以全身使用抗生素。常用的方法是阿莫西林500mg，口服，3次/日，持续10天。}此外，可以将含有强力霉素或米诺环素微球的凝胶放入孤立的顽固性囊袋中。这些药物在2周内被吸收。 第二阶段治疗是手术切除牙周袋（牙周袋缩减/清除手术）和骨成形，以便患者能够自己清洁龈沟的底部。合适的病例，进行再生手术和骨移植以促进牙槽骨生长。必须进行松动牙的夹板固定和牙齿表面选择性调磨以去除咬合创伤。\tgrn{晚期病例必须拔牙}。牙周治疗开始前控制全身性的影响因素。 90％由HIV引起的坏死溃疡性牙周炎，通过聚维酮碘牙周袋冲洗（口腔科医生用注射器处理）、经常使用氯己定漱口、适量使用抗生素（通常甲硝唑250mg，口服，3次/日，持续14天），有一定效果。 局限型侵袭性牙周炎需要牙周手术结合口服抗生素（阿莫西林500mg，4次/日，或甲硝唑250mg，3次/日，持续14日）。 \\
    \hline
    \textbf{A1 (Ours)} 牙周炎的治疗需要综合考虑危险因素、洁治和龈下刮治、口服抗生素、局部药物等多种手段。对于所有的牙周炎，第一阶段治疗包括彻底的洁治、龈下刮治和根面处理，必须加强日常的口腔卫生。\tgrn{如果存在深牙周袋，可以全身使用抗生素。常用的方法是阿莫西林500mg，口服，3次/日，持续10天。}第二阶段治疗是手术切除牙周袋和骨成形，以便患者能够自己清洁龈沟的底部。对于局限型侵袭性牙周炎需要牙周手术结合口服抗生素。同时，必须控制全身性的影响因素，如口腔卫生不良、糖尿病和吸烟，改善预后。因此，单靠药物治疗是不够的，需要综合治疗。 \\
    \hline

    \hline
    \textbf{Q2} 膝盖疼该去做什么检查？ \\
    \hline
    \textbf{{K2 (Baseline)}} \tpurp{髌腱撕裂：可触及髌骨向上方移位（高位髌骨）。 横向髌骨骨折：可触及两块碎骨之间的缝隙。 但由于局部肿胀明显，这些症状可能被误以为膝关节韧带损伤伴有关节积血。 如果患者在受伤后出现膝关节肿胀和疼痛，临床医生会要求患者坐下并尝试伸展受伤腿部以测试膝关节主动伸展或仰卧保持受伤腿部平直进行抬高。} 经验与提示 外伤后膝盖肿胀时，牢记需测试膝盖自主伸展能力。 行常规膝关节X线检查。\tpurp{膝关节X线片可以看到高位髌骨和低位髌骨。X线可显示脱位或髌骨骨折，但也可能会表现正常的。} \\
    \hline
    \textbf{K2 (Ours)} 
    % 不是每个病人都需要X线检查。然而，正位，侧位和斜位X线可用于除外骨折。渥太华膝盖规则可用于界定那些更可能患有骨折、需要特别治疗的患者。任一下列条件存在时需行X线检查：年龄＞55岁孤立的髌骨压痛（膝关节没有其他骨骼压痛）腓骨小头压痛不能屈膝90°受伤后立即无法承重，且在急诊不能完成4步行走试验，
    \tgrn{无论是否有跛行初步评估通常不需要MRI。合理的做法是保守治疗数周后症状仍没有缓解再行MRI检查。然而，严重创伤或怀疑关节内损伤，不能以其他方式排除时，还是应该行MRI。可能会进行其他测试以检查相关损伤：动脉造影或CT血管造影用于检查可疑动脉损伤。肌电图和/或神经传导检查很少直接进行，但用于损伤后数周至数月仍存在典型神经症状的患者} \\
    \hline
    \textbf{A2 (Ours)} \tgrn{对于膝盖疼痛的检查，初步评估通常不需要MRI。合理的做法是保守治疗数周后症状仍没有缓解再行MRI检查。}然而，严重创伤或怀疑关节内损伤，不能以其他方式排除时，还是应该行MRI。可能会进行其他测试以检查相关损伤，如动脉造影或CT血管造影用于检查可疑动脉损伤。肌电图和/或神经传导检查很少直接进行，但用于损伤后数周至数月仍存在典型神经症状的患者。因此，具体需要进行哪些检查，需要根据患者的具体情况而定。  \\ 
    \hline
    
  \end{tabular}
  \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
  \label{tab:example12}
\end{table*}

\begin{table*}
    \begin{tabular}{|p{\textwidth}|}
        \hline
    \textbf{Q3} 胸腔积液严重吗？ \\
    \hline
    \textbf{K3 (Baseline)} 正常情况下，脏层和壁层胸膜表面覆盖有一薄层10~20mL的胸液，其成分与血浆相似但蛋白含量较低
    （\textless 1.5g/dL[15g/l], "病因": "概述": " \tpurp{胸腔积液通常分为 漏出 渗出 积液的分类基于液体的实验室特征（请参见表 渗出性胸腔积液的判定标准 ).无论单侧或双侧，漏出液通常不需要过多的检查即可治疗，而渗出液需明确病因。多种病因可引起胸腔积液（见表 胸腔积液的病因 ）。 漏出性胸腔积液是由体循环静水压增高和血浆胶体渗透压降低引起。}  \\
    \hline
    \textbf{K3 (Ours)} \tgrn{有些胸腔积液无症状，偶然经体格检查或者胸片检查发现。大部分胸腔积液引起呼吸困难、胸膜炎性胸痛，或者二者兼有。胸膜炎性胸痛是一种模糊的不适感或者尖锐的疼痛，吸气时加重，提示壁层胸膜的炎症。疼痛感通常出现在炎症部位之上，但也可出现牵涉痛。}横膈胸膜的后部和外周部由低位的6根肋间神经支配，这些部位的刺激可引起下胸壁或腹部疼痛，表现类似腹腔内疾病。横膈胸膜的中央部分受刺激，经膈神经传导，可引起颈肩部牵涉痛。 \tgrn{体格检查示触觉语颤消失，叩诊呈浊音，积液侧呼吸音减低。胸膜增厚同样可有这些表现。}大量胸腔积液时，呼吸通常浅快。 胸膜摩擦音尽管少见，却是典型的体征。胸膜摩擦音形式多样，从类似湿啰音的间断声音到粗糙的摩擦声、嘎吱声或与呼吸同步的似皮革的声音，可在吸气相和呼气相听到。靠近心脏的摩擦音（胸膜心包摩擦音）可随心跳变化，并可能与心包炎的摩擦音混淆。心包摩擦音最佳听诊位置在胸骨左缘第三四肋间，特征为与心跳同步的来回音，并不受呼吸影响。体格检查发现胸腔积液的敏感性和特异性均较低。 \\
    \hline
    \textbf{A3 (Ours)} \tgrn{胸腔积液的严重程度需要根据患者的具体情况来判断。一般来说，大量积液会导致呼吸困难、胸痛等症状，但有些患者可能没有明显的症状。体格检查可以发现积液侧的呼吸音减低，叩诊呈浊音，同时可能出现胸膜摩擦音等体征。}但是，胸腔积液的敏感性和特异性都较低，因此需要结合临床症状和影像学检查来确定积液的严重程度和治疗方案。常见的胸腔积液病因包括心力衰竭、肺炎、结核等。    \\
    \hline
    
    \hline
    \textbf{Q4} 得了肺不张之后怎么办？\\
    \hline
    \textbf{K4 (Baseline)} 不推荐口服或静脉注射皮质类固醇，因为它们在金属烟热中没有显示出疗效。很少有既往患有肺病（如哮喘、慢性阻塞性肺病）的患者因既往疾病恶化而需要治疗和住院治疗。如果任一综合征的严重病例引起呼吸窘迫，同样 用于 ARDS 的治疗方法 （例如，机械通气、呼气末正压[PEEP]）。" , "肺不张": "概述": "\tpurp{肺不张指的是肺组织塌陷，肺容积缩小。若肺不张广泛，患者可有呼吸困难或呼吸衰竭肺。也可以发展为肺炎。肺不张通常没有明显症状，但某些情况下可能出现低氧血症和胸膜炎性胸痛。根据胸部Ｘ线片进行诊断。治疗包括保持咳嗽和深呼吸，治疗原发原因。肺不张指的是肺组织塌陷，肺容积缩小。若肺不张广泛，患者可有呼吸困难或呼吸衰竭肺。也可以发展为肺炎。肺不张通常没有明显症状，但某些情况下可能出现低氧血症和胸膜炎性胸痛。根据胸部Ｘ线片进行诊断。治疗包括保持咳嗽和深呼吸，治疗原发原因。} \\
    \hline
    \textbf{K4 (Ours)} \tgrn{保持咳嗽和深呼吸 如怀疑肿瘤或异物阻塞，需支气管镜检查 用于治疗肺不张的疗效证据均较弱或无。通常的建议包括 胸部物理治疗 ，以帮助维持肺膨胀技术，如定向咳嗽，深呼吸练习和使用的激励肺活量计的协助通气和分泌物的清除。 对于非卧床患者，锻炼（例如步行）是促进深呼吸的理想方式。} 对于未插管，分泌物不多的患者，持续气道正压可能会有帮助。对于气管插管且 机械通气 的患者，呼气末正压和/或更高的潮气量通气可能会有帮助。 避免过度镇静有助于确保通气和有效的深呼吸和咳嗽。然而，严重的胸膜疼痛可能会影响深呼吸和咳嗽，阿片类药物可协助缓解。因此，许多医生处方阿片类镇痛药用以缓解疼痛和建议患者自觉咳嗽，并定期做深呼吸。在某些病人术后，硬膜外麻醉或肋间神经阻滞可以用于缓解疼痛，而不会导致呼吸抑制。应避免镇咳。 更重要的是，针对肺不张（如粘液栓，异物，肿瘤，肿块，肺积液）的原因应及时治疗。对于持久性黏液堵塞，雾化dornase阿尔法道连酶及试用支气管扩张剂。N-Acetylcysteine通常要避免，因为它可引起支气管收缩。 如果其他措施无效或者怀疑是粘液阻塞以外的原因，应进行支气管镜检查。 \\
    \hline
    \textbf{A4 (Ours)} \tgrn{肺不张的治疗方法包括保持咳嗽和深呼吸、胸部物理治疗、锻炼、持续气道正压等。}然而，用于治疗肺不张的疗效证据不够充分，因此需要根据患者的具体情况来制定治疗方案。如果怀疑肿瘤或异物阻塞，需要进行支气管镜检查。\tgrn{对于严重的胸膜疼痛可以使用阿片类药物缓解疼痛，但应避免使用镇咳药物。}对于肺不张的病因如粘液栓、异物、肿瘤、肿块、肺积液等应有针对性的治疗。    \\
    \hline
    \end{tabular}
    \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
    \label{tab:example34}
\end{table*}
\end{CJK*}

==> tables/retrieval_cmp/retrieval_cmp_concise.tex <==

\begin{CJK*}{UTF8}{gbsn}
\begin{table*}
    \begin{tabular}{|p{\textwidth}|}
        \hline
    \textbf{Q1} Is pleural effusion serious? \\
    \hline
    \textbf{K1 (Baseline)} 
    Under normal circumstances, a thin layer of pleural fluid (10-20mL) covers the surfaces of the visceral and parietal pleura, with a composition similar to plasma but with lower protein content (\textless1.5g/dL [\textless15 g/L]). 
     \tpurp{Pleural effusions are usually classified into exudates, transudates, and fluid accumulation based on laboratory characteristics of the fluid (see criteria for diagnosing exudative pleural effusions in the table).Regardless of unilateral or bilateral involvement, leaky effusions usually require little investigation and can be treated, while exudative effusions require identification of the underlying cause. Various factors can cause pleural effusions (see the table for causes of pleural effusions). Leaky pleural effusions are caused by an increase in systemic circulatory hydrostatic pressure and a decrease in plasma colloid osmotic pressure.}  \\
    \hline
    \textbf{K1 (Ours)} 
\tgrn{Some pleural effusions are asymptomatic and are discovered incidentally during physical examination or on chest x-ray. Many cause dyspnea, pleuritic chest pain, or both. Pleuritic chest pain, a vague discomfort or sharp pain that worsens during inspiration, indicates inflammation of the parietal pleura. Pain is usually felt over the inflamed site, but referred pain is possible.} The posterior and peripheral portions of the diaphragmatic pleura are supplied by the lower 6 intercostal nerves, and irritation there may cause pain in the lower chest wall or abdomen that may simulate intra-abdominal disease. Irritation of the central portion of the diaphragmatic pleura, innervated by the phrenic nerves, causes pain referred to the neck and shoulder.
\tgrn{Physical examination reveals absent tactile fremitus, dullness to percussion, and decreased breath sounds on the side of the effusion. These findings can also be caused by pleural thickening.}

...

% With large-volume effusions, respiration is usually rapid and shallow. A pleural friction rub, although infrequent, is the classic physical sign. The friction rub varies from a few intermittent sounds that may simulate crackles to a fully developed harsh grating, creaking, or leathery sound synchronous with respiration, heard during inspiration and expiration. Friction sounds adjacent to the heart (pleuropericardial rub) may vary with the heartbeat and may be confused with the friction rub of pericarditis. 
Pericardial rub is best heard over the left border of the sternum in the 3rd and 4th intercostal spaces, is characteristically a to-and-fro sound synchronous with the heartbeat, and is not influenced significantly by respiration. Sensitivity and specificity of the physical examination for detecting effusion are probably low.\\
    \hline
    \textbf{A1 (Ours)} 
    \tgrn{The severity of pleural effusion needs to be determined based on the patient's specific situation. Generally, a large amount of effusion can cause symptoms such as dyspnea and chest pain, but some patients may not have obvious symptoms. Physical examination can reveal reduced breath sounds on the effusion side, dullness to percussion, and possibly pleural friction rub.} However, the sensitivity and specificity of physical examination for pleural effusion are both low, so clinical symptoms and imaging examinations need to be combined to determine the severity of the effusion and treatment plan. Common causes of pleural effusion include heart failure, pneumonia, and tuberculosis \\
    \hline
    
    \hline
    \textbf{Q2} What should I do after getting lung atelectasis?\\
    \hline
    \textbf{K2 (Baseline)} do not recommend oral or intravenous corticosteroids because they have not shown efficacy in metal fume fever. Patients with pre-existing lung disease (such as asthma or chronic obstructive pulmonary disease) rarely require treatment and hospitalization due to worsening of pre-existing conditions. If severe cases of either syndrome cause respiratory distress, treatment methods used for ARDS (such as mechanical ventilation and positive end-expiratory pressure [PEEP]) may also be used. "  , "Atelectasis":  "Abs": "\tpurp{Atelectasis is collapse of lung tissue with loss of volume. Patients may have dyspnea or respiratory failure if atelectasis is extensive. They may also develop pneumonia. Atelectasis is usually asymptomatic, but hypoxemia and pleuritic chest pain may be present in certain cases. Diagnosis is by chest x-ray. Treatment includes maintaining coughing and deep breathing and treating the cause."} \\
    \hline
    \textbf{K2 (Ours)} 
    \tgrn{Maximizing cough and deep breathing
    If obstruction by tumor or foreign body is suspected, bronchoscopy
Evidence for the efficacy of most treatments for atelectasis is weak or absent. Nonetheless, commonly recommended measures include chest physiotherapy to help maintain ventilation and clearance of secretions, and encouragement of lung expansion techniques such as directed cough, deep breathing exercises, and use of an incentive spirometer. In ambulatory patients, exercise (eg, walking) is a desirable way to promote deep breathing.}
For patients who are not intubated and do not have excessive secretions, continuous positive airway pressure may help. For patients who are intubated and mechanically ventilated, positive end-expiratory pressure and/or higher tidal volume ventilation may help.

...

% Avoiding oversedation helps ensure ventilation and sufficient deep breathing and coughing. However, severe pleuritic pain may impair deep breathing and coughing and may be relieved only with opioids. Thus, many clinicians prescribe opioid analgesics in doses sufficient to relieve pain and advise patients to consciously cough and take deep breaths periodically. In certain postoperative patients, epidural analgesia or an intercostal nerve block may be used to relieve pain without causing respiratory depression. Antitussive therapy should be avoided.
Most importantly, the cause of atelectasis (eg, mucous plug, foreign body, tumor, mass, pulmonary effusion) should be treated. For persistent mucous plugging, nebulized dornase alfa and sometimes bronchodilators are tried. N-Acetylcysteine is usually avoided because it can cause bronchoconstriction. 
If other measures are ineffective or if a cause of obstruction other than mucous plugging is suspected, bronchoscopy should be done.\\
    % \tgrn{保持咳嗽和深呼吸 如怀疑肿瘤或异物阻塞，需支气管镜检查 用于治疗肺不张的疗效证据均较弱或无。通常的建议包括 胸部物理治疗 ，以帮助维持肺膨胀技术，如定向咳嗽，深呼吸练习和使用的激励肺活量计的协助通气和分泌物的清除。 对于非卧床患者，锻炼（例如步行）是促进深呼吸的理想方式。} 对于未插管，分泌物不多的患者，持续气道正压可能会有帮助。对于气管插管且 机械通气 的患者，呼气末正压和/或更高的潮气量通气可能会有帮助。 避免过度镇静有助于确保通气和有效的深呼吸和咳嗽。然而，严重的胸膜疼痛可能会影响深呼吸和咳嗽，阿片类药物可协助缓解。因此，许多医生处方阿片类镇痛药用以缓解疼痛和建议患者自觉咳嗽，并定期做深呼吸。在某些病人术后，硬膜外麻醉或肋间神经阻滞可以用于缓解疼痛，而不会导致呼吸抑制。应避免镇咳。 更重要的是，针对肺不张（如粘液栓，异物，肿瘤，肿块，肺积液）的原因应及时治疗。对于持久性黏液堵塞，雾化dornase阿尔法道连酶及试用支气管扩张剂。N-Acetylcysteine通常要避免，因为它可引起支气管收缩。 如果其他措施无效或者怀疑是粘液阻塞以外的原因，应进行支气管镜检查。 \\
    \hline
    \textbf{A2 (Ours)} 
    \tgrn{The treatment methods for pulmonary atelectasis include maintaining cough and deep breathing, chest physical therapy, exercise, continuous positive airway pressure, etc.} However, the evidence for the effectiveness of these treatments is not sufficient, so the treatment plan needs to be developed according to the specific situation of the patient. If there is suspicion of tumor or foreign body obstruction, bronchoscopy examination is needed. \tgrn{Opioid drugs can be used to relieve severe pleural pain, but cough suppressant drugs should be avoided.} For the causes of pulmonary atelectasis such as mucus plugs, foreign bodies, tumors, masses, pleural effusions, etc., targeted treatments should be used.\\
    % 肺不张的治疗方法包括保持咳嗽和深呼吸、胸部物理治疗、锻炼、持续气道正压等。然而，用于治疗肺不张的疗效证据不够充分，因此需要根据患者的具体情况来制定治疗方案。如果怀疑肿瘤或异物阻塞，需要进行支气管镜检查。对于严重的胸膜疼痛可以使用阿片类药物缓解疼痛，但应避免使用镇咳药物。对于肺不张的病因如粘液栓、异物、肿瘤、肿块、肺积液等应有针对性的治疗。    \\
    \hline
    \end{tabular}
    \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
    \label{tab:example12}
\end{table*}

\begin{table*}
  \begin{tabular}{|p{\textwidth}|}
    \hline
    \textbf{Q3} How to treat periodontitis? Is taking medication enough? \\
    \hline
    \textbf{{K3 (Baseline)}} \tred{Esophageal cancer can occur at a young age. Unna-Thost disease and Vorner disease: autosomal dominant inheritance. Papillon-Lefèvre syndrome: autosomal recessive inheritance, onset within 6 months after birth. Severe periodontitis can lead to tooth loss. Vohwinkel syndrome: autosomal dominant inheritance, patients may experience progressive toe and finger amputation and high-frequency hearing loss. Diffuse non-epidermolytic palmoplantar keratoderma: this autosomal dominant inherited form develops in infancy, causing a sharply defined symmetric keratoderma affecting the entire palm and sole. Treatment: Symptomatic treatment includes the use of emollients, keratolytic agents, and physical methods for removal.} \\
    \hline
    \textbf{K3 (Ours)} 
    Treatment of risk factors
    Scaling and root planing
    \tgrn{Sometimes oral antibiotics, antibiotic packs, or both}
    Surgery or extraction
\tgrn{Treatment of modifiable risk factors such as poor oral hygiene, diabetes, and smoking improves outcomes.} 
For all forms of periodontitis, the first phase of treatment consists of thorough scaling (professional cleaning with hand or ultrasonic instruments) and root planing (removal of diseased or toxin-affected cementum and dentin followed by smoothing of the root) to remove plaque and calculus deposits. Thorough home oral hygiene is necessary and includes careful brushing and flossing to help clean. It may include chlorhexidine swabs or rinses. A therapist should help teach the patient how to do these procedures. The patient is re-evaluated after 3 weeks. If pockets are no deeper than 4 mm at this point, the only treatment needed is regular cleanings. Sometimes a flap of gum tissue is made to allow access for scaling and planing of deeper parts of the root.
\tgrn{If deeper pockets persist, systemic antibiotics can be used. A common regimen is amoxicillin 500 mg orally 3 times a day for 10 days.} In addition, a gel containing doxycycline or microspheres of minocycline can be placed into isolated recalcitrant pockets. These drugs are resorbed in 2 weeks.
Another approach is to surgically eliminate the pocket and recontour the bone (pocket reduction/elimination surgery) so that the patient can clean the depth of the normal crevice (sulcus) between the tooth and gingiva. In certain patients, regenerative surgery and bone grafting are done to encourage alveolar bone growth. Splinting of loose teeth and selective reshaping of tooth surfaces to eliminate traumatic occlusion may be necessary. \tgrn{Extractions are often necessary in advanced disease.} Contributing systemic factors should be controlled before initiating periodontal therapy.
Ninety percent of patients with necrotizing ulcerative periodontitis due to HIV (HIV-associated periodontitis) respond to combined treatment with scaling and planing, irrigation of the sulcus with povidone-iodine (which the dentist applies with a syringe), regular use of chlorhexidine mouth rinses, and systemic antibiotics, usually metronidazole 250 mg orally 3 times a day for 14 days.
Localized aggressive periodontitis requires periodontal surgery plus oral antibiotics (eg, amoxicillin 500 mg 4 times a day or metronidazole 250 mg 3 times a day for 14 days). \\
    \hline
    \textbf{A3 (Ours)} The treatment of periodontitis requires a comprehensive approach that considers risk factors, scaling and root planing, oral antibiotics, and local medications. For all cases of periodontitis, the first stage of treatment involves thorough cleaning, scaling and root planing, and reinforcement of daily oral hygiene. \tgrn{If deep periodontal pockets are present, systemic antibiotics may be used, with amoxicillin 500mg orally, three times a day for 10 days being a commonly used method.} The second stage of treatment involves surgical removal of periodontal pockets and bone reshaping to allow the patient to self-clean the base of the gingival sulcus. Localized aggressive periodontitis requires periodontal surgery in combination with oral antibiotics. At the same time, systemic factors such as poor oral hygiene, diabetes, and smoking must be controlled to improve the prognosis. Therefore, drug therapy alone is not sufficient and comprehensive treatment is necessary. \\
    \hline

    \hline
    \textbf{Q4} What tests should be done for knee pain? \\
    \hline
    \textbf{{K4 (Baseline)}} \tpurp{Patellar tendon tear: the patella is palpable and displaced upwards (high-riding patella). Transverse patellar fracture: a gap between the two pieces of the patella may be palpable. However, due to significant local swelling, these symptoms may be mistaken for knee ligament injury with joint effusion. If a patient presents with knee swelling and pain after injury, the clinician will ask the patient to sit down and attempt to extend the injured leg to test knee extension actively or lie flat and elevate the injured leg.} After knee swelling following trauma,  remember to test the knee's ability for independent extension. Routine knee joint X-ray examination should be performed. \tpurp{Knee X-rays can show a high or low position of the patella. X-rays can reveal dislocation or patellar fractures, but they may also appear normal.} \\
    \hline
    \textbf{K4 (Ours)} 
Not every patient requires x-rays. However, anteroposterior, lateral, and oblique x-rays are often taken to exclude fractures. The Ottawa knee rules are used to limit x-rays to patients more likely to have a fracture that requires specific treatments. X-rays should be taken only if one of the following is present:\\
    Age $>$ 55,\\
    Isolated tenderness of the patella (with no other bone tenderness of the knee),\\
    Tenderness of fibular head,\\
    Inability to flex the knee 90°\\
    Inability to bear weight both immediately and in the emergency department for 4 steps (with or without limping)\\
\tgrn{MRI is usually not needed at the initial evaluation. A reasonable approach is to do MRI if symptoms do not resolve after a few weeks of conservative management. However, MRI is often done when severe injury or significant intra-articular injury is suspected or cannot be otherwise excluded.
Other tests may be done to check for related injuries:
    Arteriography or CT angiography to check for suspected arterial injuries
    Electromyography and/or nerve conduction studies, which are rarely done immediately but more typically done when nerve symptoms persist weeks to months after the injury.}\\
    \hline
    \textbf{A4 (Ours)} For knee pain evaluation, \tgrn{MRI is usually not needed for initial assessment.} \tgrn{It is reasonable to proceed with conservative treatment for several weeks and perform MRI if symptoms do not improve.} However, in cases of severe trauma or suspected intra-articular injury that cannot be ruled out by other means, MRI should be performed. Other tests may be performed to investigate related injuries, such as arterial angiography or CT angiography for suspected arterial injury. Electromyography and/or nerve conduction studies are rarely performed directly, but are used for patients with typical neurological symptoms that persist for several weeks to months after injury. Therefore, which tests are needed depends on the specific situation of the patient. \\
    % 对于膝盖疼痛的检查，初步评估通常不需要MRI。合理的做法是保守治疗数周后症状仍没有缓解再行MRI检查。然而，严重创伤或怀疑关节内损伤，不能以其他方式排除时，还是应该行MRI。可能会进行其他测试以检查相关损伤，如动脉造影或CT血管造影用于检查可疑动脉损伤。肌电图和/或神经传导检查很少直接进行，但用于损伤后数周至数月仍存在典型神经症状的患者。因此，具体需要进行哪些检查，需要根据患者的具体情况而定。  \\ 
    \hline
    
  \end{tabular}
  \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
  \label{tab:example34}
\end{table*}

% \begin{table*}
%     \begin{tabular}{|p{\textwidth}|}
%         \hline
%     \textbf{Q3} Is pleural effusion serious? \\
%     \hline
%     \textbf{K3 (Baseline)} 
%     Under normal circumstances, a thin layer of pleural fluid (10-20mL) covers the surfaces of the visceral and parietal pleura, with a composition similar to plasma but with lower protein content (\textless1.5g/dL [\textless15 g/L]). 
%      \tpurp{Pleural effusions are usually classified into exudates, transudates, and fluid accumulation based on laboratory characteristics of the fluid (see criteria for diagnosing exudative pleural effusions in the table).Regardless of unilateral or bilateral involvement, leaky effusions usually require little investigation and can be treated, while exudative effusions require identification of the underlying cause. Various factors can cause pleural effusions (see the table for causes of pleural effusions). Leaky pleural effusions are caused by an increase in systemic circulatory hydrostatic pressure and a decrease in plasma colloid osmotic pressure.}  \\
%     \hline
%     \textbf{K3 (Ours)} 
% \tgrn{Some pleural effusions are asymptomatic and are discovered incidentally during physical examination or on chest x-ray. Many cause dyspnea, pleuritic chest pain, or both. Pleuritic chest pain, a vague discomfort or sharp pain that worsens during inspiration, indicates inflammation of the parietal pleura. Pain is usually felt over the inflamed site, but referred pain is possible.} The posterior and peripheral portions of the diaphragmatic pleura are supplied by the lower 6 intercostal nerves, and irritation there may cause pain in the lower chest wall or abdomen that may simulate intra-abdominal disease. Irritation of the central portion of the diaphragmatic pleura, innervated by the phrenic nerves, causes pain referred to the neck and shoulder.
% \tgrn{Physical examination reveals absent tactile fremitus, dullness to percussion, and decreased breath sounds on the side of the effusion. These findings can also be caused by pleural thickening.}

% ...

% % With large-volume effusions, respiration is usually rapid and shallow. A pleural friction rub, although infrequent, is the classic physical sign. The friction rub varies from a few intermittent sounds that may simulate crackles to a fully developed harsh grating, creaking, or leathery sound synchronous with respiration, heard during inspiration and expiration. Friction sounds adjacent to the heart (pleuropericardial rub) may vary with the heartbeat and may be confused with the friction rub of pericarditis. 
% Pericardial rub is best heard over the left border of the sternum in the 3rd and 4th intercostal spaces, is characteristically a to-and-fro sound synchronous with the heartbeat, and is not influenced significantly by respiration. Sensitivity and specificity of the physical examination for detecting effusion are probably low.\\
%     \hline
%     \textbf{A3 (Ours)} 
%     \tgrn{The severity of pleural effusion needs to be determined based on the patient's specific situation. Generally, a large amount of effusion can cause symptoms such as dyspnea and chest pain, but some patients may not have obvious symptoms. Physical examination can reveal reduced breath sounds on the effusion side, dullness to percussion, and possibly pleural friction rub.} However, the sensitivity and specificity of physical examination for pleural effusion are both low, so clinical symptoms and imaging examinations need to be combined to determine the severity of the effusion and treatment plan. Common causes of pleural effusion include heart failure, pneumonia, and tuberculosis \\
%     \hline
    
%     \hline
%     \textbf{Q4} What should I do after getting lung atelectasis?\\
%     \hline
%     \textbf{K4 (Baseline)} do not recommend oral or intravenous corticosteroids because they have not shown efficacy in metal fume fever. Patients with pre-existing lung disease (such as asthma or chronic obstructive pulmonary disease) rarely require treatment and hospitalization due to worsening of pre-existing conditions. If severe cases of either syndrome cause respiratory distress, treatment methods used for ARDS (such as mechanical ventilation and positive end-expiratory pressure [PEEP]) may also be used. "  , "Atelectasis":  "Abs": "\tpurp{Atelectasis is collapse of lung tissue with loss of volume. Patients may have dyspnea or respiratory failure if atelectasis is extensive. They may also develop pneumonia. Atelectasis is usually asymptomatic, but hypoxemia and pleuritic chest pain may be present in certain cases. Diagnosis is by chest x-ray. Treatment includes maintaining coughing and deep breathing and treating the cause."} \\
%     \hline
%     \textbf{K4 (Ours)} 
%     \tgrn{Maximizing cough and deep breathing
%     If obstruction by tumor or foreign body is suspected, bronchoscopy
% Evidence for the efficacy of most treatments for atelectasis is weak or absent. Nonetheless, commonly recommended measures include chest physiotherapy to help maintain ventilation and clearance of secretions, and encouragement of lung expansion techniques such as directed cough, deep breathing exercises, and use of an incentive spirometer. In ambulatory patients, exercise (eg, walking) is a desirable way to promote deep breathing.}
% For patients who are not intubated and do not have excessive secretions, continuous positive airway pressure may help. For patients who are intubated and mechanically ventilated, positive end-expiratory pressure and/or higher tidal volume ventilation may help.

% ...

% % Avoiding oversedation helps ensure ventilation and sufficient deep breathing and coughing. However, severe pleuritic pain may impair deep breathing and coughing and may be relieved only with opioids. Thus, many clinicians prescribe opioid analgesics in doses sufficient to relieve pain and advise patients to consciously cough and take deep breaths periodically. In certain postoperative patients, epidural analgesia or an intercostal nerve block may be used to relieve pain without causing respiratory depression. Antitussive therapy should be avoided.
% % Most importantly, the cause of atelectasis (eg, mucous plug, foreign body, tumor, mass, pulmonary effusion) should be treated. For persistent mucous plugging, nebulized dornase alfa and sometimes bronchodilators are tried. N-Acetylcysteine is usually avoided because it can cause bronchoconstriction. 
% If other measures are ineffective or if a cause of obstruction other than mucous plugging is suspected, bronchoscopy should be done.\\
%     % \tgrn{保持咳嗽和深呼吸 如怀疑肿瘤或异物阻塞，需支气管镜检查 用于治疗肺不张的疗效证据均较弱或无。通常的建议包括 胸部物理治疗 ，以帮助维持肺膨胀技术，如定向咳嗽，深呼吸练习和使用的激励肺活量计的协助通气和分泌物的清除。 对于非卧床患者，锻炼（例如步行）是促进深呼吸的理想方式。} 对于未插管，分泌物不多的患者，持续气道正压可能会有帮助。对于气管插管且 机械通气 的患者，呼气末正压和/或更高的潮气量通气可能会有帮助。 避免过度镇静有助于确保通气和有效的深呼吸和咳嗽。然而，严重的胸膜疼痛可能会影响深呼吸和咳嗽，阿片类药物可协助缓解。因此，许多医生处方阿片类镇痛药用以缓解疼痛和建议患者自觉咳嗽，并定期做深呼吸。在某些病人术后，硬膜外麻醉或肋间神经阻滞可以用于缓解疼痛，而不会导致呼吸抑制。应避免镇咳。 更重要的是，针对肺不张（如粘液栓，异物，肿瘤，肿块，肺积液）的原因应及时治疗。对于持久性黏液堵塞，雾化dornase阿尔法道连酶及试用支气管扩张剂。N-Acetylcysteine通常要避免，因为它可引起支气管收缩。 如果其他措施无效或者怀疑是粘液阻塞以外的原因，应进行支气管镜检查。 \\
%     \hline
%     \textbf{A4 (Ours)} 
%     \tgrn{The treatment methods for pulmonary atelectasis include maintaining cough and deep breathing, chest physical therapy, exercise, continuous positive airway pressure, etc.} However, the evidence for the effectiveness of these treatments is not sufficient, so the treatment plan needs to be developed according to the specific situation of the patient. If there is suspicion of tumor or foreign body obstruction, bronchoscopy examination is needed. \tgrn{Opioid drugs can be used to relieve severe pleural pain, but cough suppressant drugs should be avoided.} For the causes of pulmonary atelectasis such as mucus plugs, foreign bodies, tumors, masses, pleural effusions, etc., targeted treatments should be used.\\
%     % 肺不张的治疗方法包括保持咳嗽和深呼吸、胸部物理治疗、锻炼、持续气道正压等。然而，用于治疗肺不张的疗效证据不够充分，因此需要根据患者的具体情况来制定治疗方案。如果怀疑肿瘤或异物阻塞，需要进行支气管镜检查。对于严重的胸膜疼痛可以使用阿片类药物缓解疼痛，但应避免使用镇咳药物。对于肺不张的病因如粘液栓、异物、肿瘤、肿块、肺积液等应有针对性的治疗。    \\
%     \hline
%     \end{tabular}
%     \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
%     \label{tab:example34}
% \end{table*}
\end{CJK*}

==> tables/retrieval_cmp/retrieval_cmp_en.tex <==

\begin{CJK*}{UTF8}{gbsn}
\begin{table*}
  \begin{tabular}{|p{\textwidth}|}
    \hline
    \textbf{Q1} How to treat periodontitis? Is taking medication enough? \\
    \hline
    \textbf{{K1 (Baseline)}} \tred{Esophageal cancer can occur at a young age. Unna-Thost disease and Vorner disease: autosomal dominant inheritance. Papillon-Lefèvre syndrome: autosomal recessive inheritance, onset within 6 months after birth. Severe periodontitis can lead to tooth loss. Vohwinkel syndrome: autosomal dominant inheritance, patients may experience progressive toe and finger amputation and high-frequency hearing loss. Diffuse non-epidermolytic palmoplantar keratoderma: this autosomal dominant inherited form develops in infancy, causing a sharply defined symmetric keratoderma affecting the entire palm and sole. Treatment: Symptomatic treatment includes the use of emollients, keratolytic agents, and physical methods for removal.} \\
    \hline
    \textbf{K1 (Ours)} 
    Treatment of risk factors
    Scaling and root planing
    \tgrn{Sometimes oral antibiotics, antibiotic packs, or both}
    Surgery or extraction
\tgrn{Treatment of modifiable risk factors such as poor oral hygiene, diabetes, and smoking improves outcomes.} 

... 

% For all forms of periodontitis, the first phase of treatment consists of thorough scaling (professional cleaning with hand or ultrasonic instruments) and root planing (removal of diseased or toxin-affected cementum and dentin followed by smoothing of the root) to remove plaque and calculus deposits. Thorough home oral hygiene is necessary and includes careful brushing and flossing to help clean. It may include chlorhexidine swabs or rinses. A therapist should help teach the patient how to do these procedures. The patient is re-evaluated after 3 weeks. If pockets are no deeper than 4 mm at this point, the only treatment needed is regular cleanings. Sometimes a flap of gum tissue is made to allow access for scaling and planing of deeper parts of the root.
\tgrn{If deeper pockets persist, systemic antibiotics can be used. A common regimen is amoxicillin 500 mg orally 3 times a day for 10 days.} In addition, a gel containing doxycycline or microspheres of minocycline can be placed into isolated recalcitrant pockets. These drugs are resorbed in 2 weeks.
Another approach is to surgically eliminate the pocket and recontour the bone (pocket reduction/elimination surgery) so that the patient can clean the depth of the normal crevice (sulcus) between the tooth and gingiva. In certain patients, regenerative surgery and bone grafting are done to encourage alveolar bone growth. Splinting of loose teeth and selective reshaping of tooth surfaces to eliminate traumatic occlusion may be necessary. \tgrn{Extractions are often necessary in advanced disease.} Contributing systemic factors should be controlled before initiating periodontal therapy.
Ninety percent of patients with necrotizing ulcerative periodontitis due to HIV (HIV-associated periodontitis) respond to combined treatment with scaling and planing, irrigation of the sulcus with povidone-iodine (which the dentist applies with a syringe), regular use of chlorhexidine mouth rinses, and systemic antibiotics, usually metronidazole 250 mg orally 3 times a day for 14 days.
Localized aggressive periodontitis requires periodontal surgery plus oral antibiotics (eg, amoxicillin 500 mg 4 times a day or metronidazole 250 mg 3 times a day for 14 days). \\
    \hline
    \textbf{A1 (Ours)} The treatment of periodontitis requires a comprehensive approach that considers risk factors, scaling and root planing, oral antibiotics, and local medications. For all cases of periodontitis, the first stage of treatment involves thorough cleaning, scaling and root planing, and reinforcement of daily oral hygiene. \tgrn{If deep periodontal pockets are present, systemic antibiotics may be used, with amoxicillin 500mg orally, three times a day for 10 days being a commonly used method.} The second stage of treatment involves surgical removal of periodontal pockets and bone reshaping to allow the patient to self-clean the base of the gingival sulcus. Localized aggressive periodontitis requires periodontal surgery in combination with oral antibiotics. At the same time, systemic factors such as poor oral hygiene, diabetes, and smoking must be controlled to improve the prognosis. Therefore, drug therapy alone is not sufficient and comprehensive treatment is necessary. \\
    \hline

    \hline
    \textbf{Q2} What tests should be done for knee pain? \\
    \hline
    \textbf{{K2 (Baseline)}} \tpurp{Patellar tendon tear: the patella is palpable and displaced upwards (high-riding patella). Transverse patellar fracture: a gap between the two pieces of the patella may be palpable. However, due to significant local swelling, these symptoms may be mistaken for knee ligament injury with joint effusion. If a patient presents with knee swelling and pain after injury, the clinician will ask the patient to sit down and attempt to extend the injured leg to test knee extension actively or lie flat and elevate the injured leg.} After knee swelling following trauma,  remember to test the knee's ability for independent extension. Routine knee joint X-ray examination should be performed. \tpurp{Knee X-rays can show a high or low position of the patella. X-rays can reveal dislocation or patellar fractures, but they may also appear normal.} \\
    \hline
    \textbf{K2 (Ours)} 
% Not every patient requires x-rays. However, anteroposterior, lateral, and oblique x-rays are often taken to exclude fractures. The Ottawa knee rules are used to limit x-rays to patients more likely to have a fracture that requires specific treatments. X-rays should be taken only if one of the following is present:
%     Age > 55,
%     Isolated tenderness of the patella (with no other bone tenderness of the knee),
%     Tenderness of fibular head,
%     Inability to flex the knee 90°
%     Inability to bear weight both immediately and in the emergency department for 4 steps (with or without limping)
\tgrn{MRI is usually not needed at the initial evaluation. A reasonable approach is to do MRI if symptoms do not resolve after a few weeks of conservative management. However, MRI is often done when severe injury or significant intra-articular injury is suspected or cannot be otherwise excluded.
Other tests may be done to check for related injuries:
    Arteriography or CT angiography to check for suspected arterial injuries
    Electromyography and/or nerve conduction studies, which are rarely done immediately but more typically done when nerve symptoms persist weeks to months after the injury.}\\
    \hline
    \textbf{A2 (Ours)} For knee pain evaluation, \tgrn{MRI is usually not needed for initial assessment.} \tgrn{It is reasonable to proceed with conservative treatment for several weeks and perform MRI if symptoms do not improve.} However, in cases of severe trauma or suspected intra-articular injury that cannot be ruled out by other means, MRI should be performed. Other tests may be performed to investigate related injuries, such as arterial angiography or CT angiography for suspected arterial injury. Electromyography and/or nerve conduction studies are rarely performed directly, but are used for patients with typical neurological symptoms that persist for several weeks to months after injury. Therefore, which tests are needed depends on the specific situation of the patient. \\
    % 对于膝盖疼痛的检查，初步评估通常不需要MRI。合理的做法是保守治疗数周后症状仍没有缓解再行MRI检查。然而，严重创伤或怀疑关节内损伤，不能以其他方式排除时，还是应该行MRI。可能会进行其他测试以检查相关损伤，如动脉造影或CT血管造影用于检查可疑动脉损伤。肌电图和/或神经传导检查很少直接进行，但用于损伤后数周至数月仍存在典型神经症状的患者。因此，具体需要进行哪些检查，需要根据患者的具体情况而定。  \\ 
    \hline
    
  \end{tabular}
  \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
  \label{tab:example12}
\end{table*}

\begin{table*}
    \begin{tabular}{|p{\textwidth}|}
        \hline
    \textbf{Q3} Is pleural effusion serious? \\
    \hline
    \textbf{K3 (Baseline)} 
    Under normal circumstances, a thin layer of pleural fluid (10-20mL) covers the surfaces of the visceral and parietal pleura, with a composition similar to plasma but with lower protein content (\textless1.5g/dL [\textless15 g/L]). 
     ``Etiology'': "Abs": " \tpurp{Pleural effusions are usually classified into exudates, transudates, and fluid accumulation based on laboratory characteristics of the fluid (see criteria for diagnosing exudative pleural effusions in the table).Regardless of unilateral or bilateral involvement, leaky effusions usually require little investigation and can be treated, while exudative effusions require identification of the underlying cause. Various factors can cause pleural effusions (see the table for causes of pleural effusions). Leaky pleural effusions are caused by an increase in systemic circulatory hydrostatic pressure and a decrease in plasma colloid osmotic pressure.}  \\
    \hline
    \textbf{K3 (Ours)} 
\tgrn{Some pleural effusions are asymptomatic and are discovered incidentally during physical examination or on chest x-ray. Many cause dyspnea, pleuritic chest pain, or both. Pleuritic chest pain, a vague discomfort or sharp pain that worsens during inspiration, indicates inflammation of the parietal pleura. Pain is usually felt over the inflamed site, but referred pain is possible.} The posterior and peripheral portions of the diaphragmatic pleura are supplied by the lower 6 intercostal nerves, and irritation there may cause pain in the lower chest wall or abdomen that may simulate intra-abdominal disease. Irritation of the central portion of the diaphragmatic pleura, innervated by the phrenic nerves, causes pain referred to the neck and shoulder.
\tgrn{Physical examination reveals absent tactile fremitus, dullness to percussion, and decreased breath sounds on the side of the effusion. These findings can also be caused by pleural thickening.}

...

% With large-volume effusions, respiration is usually rapid and shallow. A pleural friction rub, although infrequent, is the classic physical sign. The friction rub varies from a few intermittent sounds that may simulate crackles to a fully developed harsh grating, creaking, or leathery sound synchronous with respiration, heard during inspiration and expiration. Friction sounds adjacent to the heart (pleuropericardial rub) may vary with the heartbeat and may be confused with the friction rub of pericarditis. 
Pericardial rub is best heard over the left border of the sternum in the 3rd and 4th intercostal spaces, is characteristically a to-and-fro sound synchronous with the heartbeat, and is not influenced significantly by respiration. Sensitivity and specificity of the physical examination for detecting effusion are probably low.\\
    \hline
    \textbf{A3 (Ours)} 
    \tgrn{The severity of pleural effusion needs to be determined based on the patient's specific situation. Generally, a large amount of effusion can cause symptoms such as dyspnea and chest pain, but some patients may not have obvious symptoms. Physical examination can reveal reduced breath sounds on the effusion side, dullness to percussion, and possibly pleural friction rub.} However, the sensitivity and specificity of physical examination for pleural effusion are both low, so clinical symptoms and imaging examinations need to be combined to determine the severity of the effusion and treatment plan. Common causes of pleural effusion include heart failure, pneumonia, and tuberculosis \\
    \hline
    
    \hline
    \textbf{Q4} What should I do after getting lung atelectasis?\\
    \hline
    \textbf{K4 (Baseline)} do not recommend oral or intravenous corticosteroids because they have not shown efficacy in metal fume fever. Patients with pre-existing lung disease (such as asthma or chronic obstructive pulmonary disease) rarely require treatment and hospitalization due to worsening of pre-existing conditions. If severe cases of either syndrome cause respiratory distress, treatment methods used for ARDS (such as mechanical ventilation and positive end-expiratory pressure [PEEP]) may also be used. "  , "Atelectasis":  "Abs": "\tpurp{Atelectasis is collapse of lung tissue with loss of volume. Patients may have dyspnea or respiratory failure if atelectasis is extensive. They may also develop pneumonia. Atelectasis is usually asymptomatic, but hypoxemia and pleuritic chest pain may be present in certain cases. Diagnosis is by chest x-ray. Treatment includes maintaining coughing and deep breathing and treating the cause."} \\
    \hline
    \textbf{K4 (Ours)} 
    \tgrn{Maximizing cough and deep breathing
    If obstruction by tumor or foreign body is suspected, bronchoscopy
Evidence for the efficacy of most treatments for atelectasis is weak or absent. Nonetheless, commonly recommended measures include chest physiotherapy to help maintain ventilation and clearance of secretions, and encouragement of lung expansion techniques such as directed cough, deep breathing exercises, and use of an incentive spirometer. In ambulatory patients, exercise (eg, walking) is a desirable way to promote deep breathing.}
For patients who are not intubated and do not have excessive secretions, continuous positive airway pressure may help. For patients who are intubated and mechanically ventilated, positive end-expiratory pressure and/or higher tidal volume ventilation may help.

...

% Avoiding oversedation helps ensure ventilation and sufficient deep breathing and coughing. However, severe pleuritic pain may impair deep breathing and coughing and may be relieved only with opioids. Thus, many clinicians prescribe opioid analgesics in doses sufficient to relieve pain and advise patients to consciously cough and take deep breaths periodically. In certain postoperative patients, epidural analgesia or an intercostal nerve block may be used to relieve pain without causing respiratory depression. Antitussive therapy should be avoided.
% Most importantly, the cause of atelectasis (eg, mucous plug, foreign body, tumor, mass, pulmonary effusion) should be treated. For persistent mucous plugging, nebulized dornase alfa and sometimes bronchodilators are tried. N-Acetylcysteine is usually avoided because it can cause bronchoconstriction. 
If other measures are ineffective or if a cause of obstruction other than mucous plugging is suspected, bronchoscopy should be done.\\
    % \tgrn{保持咳嗽和深呼吸 如怀疑肿瘤或异物阻塞，需支气管镜检查 用于治疗肺不张的疗效证据均较弱或无。通常的建议包括 胸部物理治疗 ，以帮助维持肺膨胀技术，如定向咳嗽，深呼吸练习和使用的激励肺活量计的协助通气和分泌物的清除。 对于非卧床患者，锻炼（例如步行）是促进深呼吸的理想方式。} 对于未插管，分泌物不多的患者，持续气道正压可能会有帮助。对于气管插管且 机械通气 的患者，呼气末正压和/或更高的潮气量通气可能会有帮助。 避免过度镇静有助于确保通气和有效的深呼吸和咳嗽。然而，严重的胸膜疼痛可能会影响深呼吸和咳嗽，阿片类药物可协助缓解。因此，许多医生处方阿片类镇痛药用以缓解疼痛和建议患者自觉咳嗽，并定期做深呼吸。在某些病人术后，硬膜外麻醉或肋间神经阻滞可以用于缓解疼痛，而不会导致呼吸抑制。应避免镇咳。 更重要的是，针对肺不张（如粘液栓，异物，肿瘤，肿块，肺积液）的原因应及时治疗。对于持久性黏液堵塞，雾化dornase阿尔法道连酶及试用支气管扩张剂。N-Acetylcysteine通常要避免，因为它可引起支气管收缩。 如果其他措施无效或者怀疑是粘液阻塞以外的原因，应进行支气管镜检查。 \\
    \hline
    \textbf{A4 (Ours)} 
    \tgrn{The treatment methods for pulmonary atelectasis include maintaining cough and deep breathing, chest physical therapy, exercise, continuous positive airway pressure, etc.} However, the evidence for the effectiveness of these treatments is not sufficient, so the treatment plan needs to be developed according to the specific situation of the patient. If there is suspicion of tumor or foreign body obstruction, bronchoscopy examination is needed. \tgrn{Opioid drugs can be used to relieve severe pleural pain, but cough suppressant drugs should be avoided.} For the causes of pulmonary atelectasis such as mucus plugs, foreign bodies, tumors, masses, pleural effusions, etc., targeted treatments should be used.\\
    % 肺不张的治疗方法包括保持咳嗽和深呼吸、胸部物理治疗、锻炼、持续气道正压等。然而，用于治疗肺不张的疗效证据不够充分，因此需要根据患者的具体情况来制定治疗方案。如果怀疑肿瘤或异物阻塞，需要进行支气管镜检查。对于严重的胸膜疼痛可以使用阿片类药物缓解疼痛，但应避免使用镇咳药物。对于肺不张的病因如粘液栓、异物、肿瘤、肿块、肺积液等应有针对性的治疗。    \\
    \hline
    \end{tabular}
    \caption{Comparison between knowledge retrieval methods. Completely unrelated knowledge is marked in \tred{red}, partially related knowledge is  marked in \tpurp{purple}. Related and important knowledge is in \tgrn{green}.}
    \label{tab:example34}
\end{table*}
\end{CJK*}

==> tables/revised_baseline.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{lrrrrrrrrrrr}
    \toprule
    Model & \multicolumn{1}{l}{Size} & \multicolumn{1}{l}{C-BLEU} & \multicolumn{1}{l}{BLEU-1} & \multicolumn{1}{l}{BLEU-2} & \multicolumn{1}{l}{BLEU-3} & \multicolumn{1}{l}{BLEU-4} & \multicolumn{1}{l}{ROUGE-L} & \multicolumn{1}{l}{METEOR} & \multicolumn{1}{l}{PRE} & \multicolumn{1}{l}{REC} & \multicolumn{1}{l}{F1} \\
    \midrule
    R2GenCMN &       &       &       &       &       &       &       &       &       &       &  \\
    VLCI  &       &       &       &       &       &       &       &       &       &       &  \\
    ChatCAD (P3) &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    ChatCAD+ (P1) &       &       &       &       &       &       &       &       & \multicolumn{1}{l}{0.548} & \multicolumn{1}{l}{0.484} & \multicolumn{1}{l}{0.502} \\
    ChatCAD+ (P2) &       &       &       &       &       &       &       &       & \multicolumn{1}{l}{0.538} & \multicolumn{1}{l}{0.597} & \multicolumn{1}{l}{0.557} \\
    ChatCAD+ (P3) &       &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:revised_baseline}%
\end{table}%

